Discovery of the Optical Counterparts to Four Energetic Fermi Millisecond Pulsars

In the last few years, over 43 millisecond radio pulsars have been discovered by targeted searches of unidentified gamma-ray sources found by the Fermi Gamma-Ray Space Telescope. A large fraction of these millisecond pulsars are in compact binaries with low-mass companions. These systems often show eclipses of the pulsar signal and are commonly known as black widows and redbacks because the pulsar is gradually destroying its companion. In this paper, we report on the optical discovery of four strongly irradiated millisecond pulsar companions. All four sources show modulations of their color and luminosity at the known orbital periods from radio timing. Light curve modelling of our exploratory data shows that the equilibrium temperature reached on the companion's dayside with respect to their nightside is consistent with about 10-30% of the available spin-down energy from the pulsar being reprocessed to increase the companion's dayside temperature. This value compares well with the range observed in other irradiated pulsar binaries and offers insights about the energetics of the pulsar wind and the production of gamma-ray emission. In addition, this provides a simple way of estimating the brightness of irradiated pulsar companions given the pulsar spin-down luminosity. Our analysis also suggests that two of the four new irradiated pulsar companions are only partially filling their Roche lobe. Some of these sources are relatively bright and represent good targets for spectroscopic follow-up. These measurements could enable, among other things, mass determination of the neutron stars in these systems.

==> online_tables.tex <==

\begin{table}[!ht]
\begin{center}
\caption{Photometry of PSR~J0023+09's Field}
\begin{tabular}{cccccccccc}
\hline
\hline
RA & Dec & $F_g$ & $\delta_{F_g}$ & $F_i$ & $\delta_{F_i}$ & $g$ Mag.\tablenotemark{a} & $g$ Mag. Error\tablenotemark{b} & $i$ Mag. \tablenotemark{a} & $i$ Mag. Error\tablenotemark{b} \\
 ($^\circ$) & ($^\circ$) & ($\mu Jy$) & ($\mu Jy$) & ($\mu Jy$) & ($\mu Jy$) &  &  & &  \\
\hline
5.8186 & 9.33167 & 17.866 & 0.461 & 37.066 & 14.874 & 20.770 & 0.028 & 19.977 & 0.436 \\
5.8316 & 9.32724 & 43.987 & 5.481 & 531.848 & 275.488 & 19.791 & 0.135 & 17.085 & 0.562 \\
5.8362 & 9.32149 & 13.635 & 0.354 & 169.842 & 69.976 & 21.063 & 0.028 & 18.325 & 0.447 \\
5.8478 & 9.30288 & 26.704 & 0.680 & 202.056 & 88.088 & 20.333 & 0.028 & 18.136 & 0.473 \\
\end{tabular}\label{t:cat_j0023}
\tablenotetext{1}{AB magnitudes in the Lupton system, $m = m_{_0} - 2.5 \log b^\prime - (2.5 \log e) \sinh^{-1} (f/2b^\prime)$, using softening parameters $b^\prime = 0.059$ and 0.233 $\mu Jy$ for the $g$ and $i$ band, respectively, and zeropoint $m_{_0} = -48.6$.}
\tablenotetext{2}{The flux and magnitude errors represent the formal uncertainties. One should also add in quadrature the zeropoint calibration errors, which are 0.319 and 0.757 mag in $g$ and $i$ band, respectively.}
\end{center}
\end{table}

\begin{table}[!ht]
\begin{center}
\caption{Photometry of PSR~J2256$-$10's Field}
\begin{tabular}{cccccccccc}
\hline
\hline
RA & Dec & $F_g$ & $\delta_{F_g}$ & $F_i$ & $\delta_{F_i}$ & $g$ Mag.\tablenotemark{a} & $g$ Mag. Error\tablenotemark{b} & $i$ Mag. \tablenotemark{a} & $i$ Mag. Error\tablenotemark{b} \\
 ($^\circ$) & ($^\circ$) & ($\mu Jy$) & ($\mu Jy$) & ($\mu Jy$) & ($\mu Jy$) &  &  & &  \\
\hline
344.2510 & -10.42511 & 22.727 & 0.217 & 38.130 & 2.082 & 20.508 & 0.010 & 19.947 & 0.059 \\
344.2164 & -10.44467 & 77.142 & 0.666 & 141.237 & 9.110 & 19.182 & 0.009 & 18.525 & 0.070 \\
344.2267 & -10.44734 & 45.995 & 0.544 & 52.843 & 3.538 & 19.743 & 0.013 & 19.592 & 0.073 \\
344.2162 & -10.45483 & 32.540 & 0.227 & 162.944 & 11.661 & 20.119 & 0.008 & 18.370 & 0.078 \\
\end{tabular}\label{t:cat_j2256}
\tablenotetext{1}{AB magnitudes in the Lupton system, $m = m_{_0} - 2.5 \log b^\prime - (2.5 \log e) \sinh^{-1} (f/2b^\prime)$, using softening parameters $b^\prime = 0.025$ and 0.064 $\mu Jy$ for the $g$ and $i$ band, respectively, and zeropoint $m_{_0} = -48.6$.}
\tablenotetext{2}{The flux and magnitude errors represent the formal uncertainties. One should also add in quadrature the zeropoint calibration errors, which are 0.104 and 0.119 mag in $g$ and $i$ band, respectively.}
\end{center}
\end{table}

\begin{table}[!ht]
\begin{center}
\caption{Photometry of PSR~J1810+17's Field}
\begin{tabular}{cccccccccc}
\hline
\hline
RA & Dec & $F_g$ & $\delta_{F_g}$ & $F_i$ & $\delta_{F_i}$ & $g$ Mag.\tablenotemark{a} & $g$ Mag. Error\tablenotemark{b} & $i$ Mag. \tablenotemark{a} & $i$ Mag. Error\tablenotemark{b} \\
 ($^\circ$) & ($^\circ$) & ($\mu Jy$) & ($\mu Jy$) & ($\mu Jy$) & ($\mu Jy$) &  &  & &  \\
\hline
272.6369 & 17.69634 & 237.271 & 2.411 & 346.437 & 27.159 & 17.962 & 0.011 & 17.551 & 0.085 \\
272.6447 & 17.69635 & 103.994 & 1.271 & 326.656 & 28.107 & 18.857 & 0.013 & 17.615 & 0.093 \\
272.6412 & 17.69643 & 13.180 & 0.089 & 84.170 & 1.248 & 21.100 & 0.007 & 19.087 & 0.016 \\
272.6556 & 17.69722 & 19.951 & 0.185 & 27.200 & 0.387 & 20.650 & 0.010 & 20.313 & 0.015 \\
272.6356 & 17.70056 & 19.121 & 0.141 & 47.389 & 0.649 & 20.696 & 0.008 & 19.711 & 0.015 \\
272.6364 & 17.70069 & 51.520 & 0.717 & 177.080 & 4.442 & 19.620 & 0.015 & 18.279 & 0.027 \\
272.6494 & 17.70144 & 39.682 & 0.399 & 46.183 & 0.621 & 19.903 & 0.011 & 19.739 & 0.015 \\
272.6288 & 17.70616 & 252.172 & 1.541 & 267.354 & 12.181 & 17.896 & 0.007 & 17.832 & 0.049 \\
272.6511 & 17.70718 & 129.106 & 0.860 & 194.194 & 5.148 & 18.622 & 0.007 & 18.179 & 0.029 \\
272.6253 & 17.70829 & 21.992 & 0.280 & 147.220 & 1.716 & 20.544 & 0.014 & 18.480 & 0.013 \\
272.6321 & 17.70842 & 112.807 & 0.668 & 131.862 & 3.092 & 18.769 & 0.006 & 18.599 & 0.025 \\
272.6541 & 17.70913 & 70.777 & 0.663 & 109.844 & 2.282 & 19.275 & 0.010 & 18.798 & 0.023 \\
272.6412 & 17.70941 & 15.921 & 0.104 & 24.255 & 0.269 & 20.895 & 0.007 & 20.438 & 0.012 \\
272.6270 & 17.71032 & 101.868 & 1.126 & 137.046 & 2.427 & 18.880 & 0.012 & 18.558 & 0.019 \\
272.6621 & 17.71082 & 22.163 & 0.214 & 35.364 & 0.643 & 20.536 & 0.010 & 20.028 & 0.020 \\
272.6259 & 17.71213 & 24.799 & 0.312 & 73.268 & 1.337 & 20.414 & 0.014 & 19.237 & 0.020 \\
272.6410 & 17.71220 & 12.695 & 0.160 & 25.094 & 0.384 & 21.141 & 0.014 & 20.401 & 0.017 \\
272.6428 & 17.71452 & 20.762 & 0.170 & 41.949 & 0.548 & 20.607 & 0.009 & 19.843 & 0.014 \\
272.6313 & 17.71464 & 108.574 & 1.512 & 141.178 & 1.716 & 18.810 & 0.015 & 18.525 & 0.013 \\
272.6620 & 17.71502 & 72.208 & 0.736 & 107.341 & 1.642 & 19.253 & 0.011 & 18.823 & 0.017 \\
272.6544 & 17.71546 & 31.512 & 0.279 & 194.513 & 7.053 & 20.154 & 0.010 & 18.177 & 0.039 \\
272.6576 & 17.71613 & 57.833 & 0.636 & 228.220 & 11.228 & 19.494 & 0.012 & 18.004 & 0.053 \\
272.6552 & 17.71629 & 33.000 & 0.253 & 229.159 & 10.828 & 20.103 & 0.008 & 17.999 & 0.051 \\
272.6475 & 17.71824 & 18.332 & 0.298 & 142.936 & 2.924 & 20.742 & 0.018 & 18.512 & 0.022 \\
272.6455 & 17.71847 & 25.035 & 0.149 & 34.625 & 0.397 & 20.403 & 0.006 & 20.051 & 0.012 \\
272.6502 & 17.71874 & 66.459 & 0.428 & 116.147 & 2.016 & 19.343 & 0.007 & 18.737 & 0.019 \\
272.6376 & 17.71905 & 19.083 & 0.131 & 34.859 & 0.489 & 20.698 & 0.007 & 20.044 & 0.015 \\
272.6624 & 17.72009 & 92.576 & 0.916 & 144.691 & 2.387 & 18.984 & 0.011 & 18.499 & 0.018 \\
272.6599 & 17.72052 & 188.783 & 1.086 & 244.937 & 13.326 & 18.210 & 0.006 & 17.927 & 0.059 \\
272.6275 & 17.72063 & 64.352 & 0.868 & 113.230 & 1.430 & 19.378 & 0.015 & 18.765 & 0.014 \\
272.6470 & 17.72063 & 16.413 & 0.099 & 44.597 & 0.825 & 20.862 & 0.007 & 19.776 & 0.020 \\
272.6415 & 17.72187 & 76.144 & 1.067 & 137.140 & 1.910 & 19.196 & 0.015 & 18.557 & 0.015 \\
272.6288 & 17.72262 & 22.705 & 0.160 & 44.961 & 0.598 & 20.509 & 0.008 & 19.768 & 0.014 \\
272.6557 & 17.72264 & 22.560 & 0.240 & 33.821 & 0.715 & 20.516 & 0.012 & 20.077 & 0.023 \\
272.6384 & 17.72281 & 40.423 & 0.467 & 68.717 & 0.767 & 19.883 & 0.013 & 19.307 & 0.012 \\
272.6347 & 17.72355 & 82.855 & 0.778 & 141.207 & 2.422 & 19.104 & 0.010 & 18.525 & 0.019 \\
272.6451 & 17.72381 & 111.895 & 0.883 & 166.465 & 5.194 & 18.778 & 0.009 & 18.346 & 0.034 \\
272.6443 & 17.72411 & 41.254 & 0.438 & 71.886 & 1.149 & 19.861 & 0.012 & 19.258 & 0.017 \\
272.6335 & 17.72487 & 47.742 & 0.475 & 80.574 & 1.401 & 19.703 & 0.011 & 19.134 & 0.019 \\
272.6366 & 17.72626 & 13.572 & 0.094 & 49.953 & 0.846 & 21.068 & 0.008 & 19.653 & 0.018 \\
272.6501 & 17.72653 & 21.831 & 0.201 & 92.726 & 1.640 & 20.552 & 0.010 & 18.982 & 0.019 \\
272.6590 & 17.72652 & 18.480 & 0.168 & 103.358 & 1.669 & 20.733 & 0.010 & 18.864 & 0.018 \\
272.6621 & 17.72855 & 18.525 & 0.175 & 146.208 & 2.617 & 20.730 & 0.010 & 18.487 & 0.019 \\
272.6258 & 17.73086 & 146.758 & 0.861 & 184.880 & 3.849 & 18.483 & 0.006 & 18.233 & 0.023 \\
272.6619 & 17.73278 & 22.832 & 0.252 & 36.467 & 1.034 & 20.503 & 0.012 & 19.995 & 0.031 \\
272.6447 & 17.73352 & 40.993 & 0.441 & 107.575 & 1.594 & 19.868 & 0.012 & 18.820 & 0.016 \\
272.6653 & 17.73520 & 17.554 & 0.114 & 51.796 & 0.688 & 20.789 & 0.007 & 19.614 & 0.014 \\
272.6291 & 17.73686 & 13.244 & 0.143 & 14.963 & 0.264 & 21.095 & 0.012 & 20.962 & 0.019 \\
272.6441 & 17.73757 & 206.874 & 1.983 & 235.076 & 14.220 & 18.111 & 0.010 & 17.972 & 0.066 \\
272.6467 & 17.73845 & 34.669 & 0.327 & 58.845 & 0.749 & 20.050 & 0.010 & 19.475 & 0.014 \\
272.6385 & 17.74117 & 24.700 & 0.184 & 44.164 & 0.628 & 20.418 & 0.008 & 19.787 & 0.015 \\
272.6339 & 17.74119 & 46.137 & 0.459 & 114.033 & 1.708 & 19.740 & 0.011 & 18.757 & 0.016 \\
272.6395 & 17.74283 & 12.626 & 0.127 & 60.396 & 1.037 & 21.147 & 0.011 & 19.447 & 0.019 \\
272.6473 & 17.74315 & 12.260 & 0.100 & 115.603 & 1.722 & 21.179 & 0.009 & 18.742 & 0.016 \\
272.6663 & 17.74534 & 25.683 & 0.246 & 51.918 & 1.235 & 20.376 & 0.010 & 19.611 & 0.026 \\
272.6281 & 17.74542 & 16.287 & 0.151 & 124.498 & 2.403 & 20.870 & 0.010 & 18.662 & 0.021 \\
272.6340 & 17.74575 & 66.306 & 0.665 & 98.876 & 1.432 & 19.346 & 0.011 & 18.912 & 0.016 \\
272.6547 & 17.74630 & 12.566 & 0.114 & 32.198 & 0.498 & 21.152 & 0.010 & 20.130 & 0.017 \\
272.6256 & 17.74767 & 108.580 & 1.051 & 261.808 & 16.149 & 18.810 & 0.011 & 17.855 & 0.067 \\
272.6489 & 17.74804 & 133.662 & 1.465 & 189.407 & 8.186 & 18.585 & 0.012 & 18.206 & 0.047 \\
272.6381 & 17.74856 & 89.828 & 0.545 & 135.181 & 2.244 & 19.016 & 0.007 & 18.572 & 0.018 \\
272.6267 & 17.74928 & 38.717 & 0.236 & 92.716 & 1.333 & 19.930 & 0.007 & 18.982 & 0.016 \\
272.6396 & 17.75022 & 20.341 & 0.216 & 31.446 & 0.643 & 20.629 & 0.012 & 20.156 & 0.022 \\
272.6489 & 17.75036 & 17.664 & 0.140 & 28.985 & 0.363 & 20.782 & 0.009 & 20.244 & 0.014 \\
272.6305 & 17.75158 & 12.890 & 0.120 & 101.235 & 1.418 & 21.124 & 0.010 & 18.886 & 0.015 \\
272.6315 & 17.75292 & 32.740 & 0.334 & 44.444 & 0.943 & 20.112 & 0.011 & 19.780 & 0.023 \\
272.6436 & 17.75327 & 46.422 & 0.342 & 62.817 & 0.838 & 19.733 & 0.008 & 19.405 & 0.014 \\
272.6633 & 17.75538 & 31.986 & 0.205 & 192.732 & 7.549 & 20.137 & 0.007 & 18.187 & 0.043 \\
272.6653 & 17.75569 & 40.908 & 0.265 & 137.909 & 2.599 & 19.870 & 0.007 & 18.551 & 0.020 \\
272.6371 & 17.75959 & 67.403 & 0.711 & 105.967 & 1.741 & 19.328 & 0.011 & 18.837 & 0.018 \\
272.6665 & 17.76025 & 10.586 & 0.123 & 29.225 & 0.314 & 21.338 & 0.013 & 20.235 & 0.012 \\
272.6295 & 17.76141 & 25.776 & 0.203 & 44.641 & 0.566 & 20.372 & 0.009 & 19.775 & 0.014 \\
272.6664 & 17.76177 & 25.283 & 0.893 & 39.034 & 1.104 & 20.393 & 0.038 & 19.921 & 0.031 \\
272.6569 & 17.76206 & 140.935 & 0.853 & 271.441 & 20.193 & 18.527 & 0.007 & 17.816 & 0.081 \\
272.6663 & 17.76218 & 50.596 & 0.558 & 61.725 & 0.793 & 19.639 & 0.012 & 19.424 & 0.014 \\
272.6391 & 17.76222 & 22.372 & 0.227 & 38.082 & 0.498 & 20.526 & 0.011 & 19.948 & 0.014 \\
272.6558 & 17.76232 & 31.070 & 0.274 & 54.174 & 0.877 & 20.169 & 0.010 & 19.565 & 0.018 \\
272.6368 & 17.76340 & 26.812 & 0.201 & 119.491 & 2.242 & 20.329 & 0.008 & 18.706 & 0.020 \\
272.6252 & 17.76357 & 37.777 & 0.312 & 53.520 & 0.810 & 19.957 & 0.009 & 19.578 & 0.016 \\
272.6503 & 17.76646 & 31.886 & 0.354 & 60.128 & 1.407 & 20.141 & 0.012 & 19.452 & 0.025 \\
272.6272 & 17.76798 & 58.114 & 0.397 & 73.041 & 1.181 & 19.489 & 0.007 & 19.241 & 0.018 \\
272.6536 & 17.76819 & 14.368 & 0.114 & 21.267 & 0.255 & 21.006 & 0.009 & 20.580 & 0.013 \\
272.6638 & 17.77141 & 23.966 & 0.157 & 47.707 & 0.539 & 20.451 & 0.007 & 19.703 & 0.012 \\
272.6580 & 17.77272 & 13.560 & 0.118 & 42.596 & 0.784 & 21.069 & 0.009 & 19.826 & 0.020 \\
272.6554 & 17.77340 & 18.051 & 0.132 & 83.933 & 1.225 & 20.759 & 0.008 & 19.090 & 0.016 \\
272.6554 & 17.77485 & 13.317 & 0.113 & 102.249 & 1.327 & 21.089 & 0.009 & 18.876 & 0.014 \\
272.6466 & 17.77561 & 29.008 & 0.211 & 41.672 & 0.828 & 20.243 & 0.008 & 19.850 & 0.022 \\
272.6254 & 17.77579 & 89.180 & 0.758 & 277.645 & 15.600 & 19.024 & 0.009 & 17.791 & 0.061 \\
272.6539 & 17.77698 & 13.445 & 0.136 & 38.077 & 0.672 & 21.078 & 0.011 & 19.948 & 0.019 \\
272.6476 & 17.77767 & 86.718 & 0.596 & 147.721 & 2.789 & 19.054 & 0.007 & 18.476 & 0.021 \\
272.6537 & 17.77769 & 22.912 & 0.186 & 53.420 & 0.686 & 20.500 & 0.009 & 19.581 & 0.014 \\
272.6337 & 17.78091 & 24.391 & 0.201 & 44.502 & 0.836 & 20.432 & 0.009 & 19.779 & 0.020 \\
272.6663 & 17.78115 & 22.866 & 0.168 & 91.372 & 1.288 & 20.502 & 0.008 & 18.998 & 0.015 \\
272.6346 & 17.78338 & 17.473 & 0.201 & 75.224 & 1.730 & 20.794 & 0.013 & 19.209 & 0.025 \\
272.6618 & 17.78340 & 26.646 & 0.248 & 93.114 & 1.657 & 20.336 & 0.010 & 18.977 & 0.019 \\
272.6430 & 17.78458 & 108.859 & 0.893 & 169.375 & 3.489 & 18.808 & 0.009 & 18.328 & 0.022 \\
272.6634 & 17.78552 & 21.268 & 0.407 & 45.762 & 0.899 & 20.580 & 0.021 & 19.748 & 0.021 \\
272.6627 & 17.78563 & 32.704 & 0.317 & 47.525 & 1.168 & 20.113 & 0.011 & 19.707 & 0.027 \\
272.6303 & 17.78592 & 12.939 & 0.077 & 39.508 & 0.705 & 21.120 & 0.006 & 19.908 & 0.019 \\
272.6627 & 17.78638 & 37.240 & 0.366 & 74.095 & 0.929 & 19.972 & 0.011 & 19.225 & 0.014 \\
\end{tabular}\label{t:cat_j1810}
\tablenotetext{1}{AB magnitudes in the Lupton system, $m = m_{_0} - 2.5 \log b^\prime - (2.5 \log e) \sinh^{-1} (f/2b^\prime)$, using softening parameters $b^\prime = 0.051$ and 0.099 $\mu Jy$ for the $g$ and $i$ band, respectively, and zeropoint $m_{_0} = -48.6$.}
\tablenotetext{2}{The flux and magnitude errors represent the formal uncertainties. One should also add in quadrature the zeropoint calibration errors, which are 0.301 and 0.308 mag in $g$ and $i$ band, respectively.}
\end{center}
\end{table}

\begin{table}[!ht]
\begin{center}
\caption{Photometry of PSR~J2215+51's Field}
\begin{tabular}{cccccccccc}
\hline
\hline
RA & Dec & $F_g$ & $\delta_{F_g}$ & $F_i$ & $\delta_{F_i}$ & $g$ Mag.\tablenotemark{a} & $g$ Mag. Error\tablenotemark{b} & $i$ Mag. \tablenotemark{a} & $i$ Mag. Error\tablenotemark{b} \\
 ($^\circ$) & ($^\circ$) & ($\mu Jy$) & ($\mu Jy$) & ($\mu Jy$) & ($\mu Jy$) &  &  & &  \\
\hline
333.8574 & 51.63511 & 221.536 & 3.620 & 373.948 & 4.511 & 18.0362 & 0.0177 & 17.468 & 0.013 \\
333.8495 & 51.63287 & 198.380 & 3.408 & 226.192 & 5.533 & 18.1560 & 0.0187 & 18.014 & 0.027 \\
333.8788 & 51.63873 & 277.515 & 4.527 & 312.974 & 3.977 & 17.7915 & 0.0177 & 17.661 & 0.014 \\
333.8647 & 51.63464 & 146.872 & 2.404 & 226.669 & 3.481 & 18.4824 & 0.0178 & 18.011 & 0.017 \\
333.8832 & 51.63762 & 200.902 & 3.290 & 301.990 & 3.080 & 18.1423 & 0.0178 & 17.700 & 0.011 \\
333.8814 & 51.63701 & 164.130 & 2.681 & 249.600 & 6.743 & 18.3618 & 0.0177 & 17.907 & 0.029 \\
333.8661 & 51.63308 & 73.223 & 1.197 & 162.063 & 1.875 & 19.2381 & 0.0177 & 18.376 & 0.013 \\
333.8700 & 51.63366 & 45.210 & 0.744 & 126.872 & 0.440 & 19.7616 & 0.0179 & 18.641 & 0.004 \\
333.8784 & 51.63521 & 193.963 & 3.170 & 260.084 & 2.634 & 18.1805 & 0.0177 & 17.862 & 0.011 \\
333.8706 & 51.63297 & 21.824 & 0.463 & 88.451 & 2.139 & 20.5523 & 0.0230 & 19.033 & 0.026 \\
333.8633 & 51.63074 & 466.213 & 7.600 & 508.156 & 5.820 & 17.2283 & 0.0177 & 17.135 & 0.012 \\
333.8489 & 51.62594 & 397.258 & 6.496 & 479.093 & 6.206 & 17.4021 & 0.0178 & 17.199 & 0.014 \\
333.8868 & 51.63390 & 437.076 & 7.136 & 494.698 & 5.382 & 17.2984 & 0.0177 & 17.164 & 0.012 \\
333.8648 & 51.62868 & 116.373 & 1.899 & 191.563 & 1.127 & 18.7351 & 0.0177 & 18.194 & 0.006 \\
333.8365 & 51.62103 & 27.941 & 0.460 & 125.100 & 1.332 & 20.2841 & 0.0179 & 18.657 & 0.012 \\
333.8665 & 51.62695 & 25.405 & 0.419 & 119.691 & 1.281 & 20.3873 & 0.0179 & 18.705 & 0.012 \\
333.8872 & 51.63079 & 289.371 & 4.722 & 342.334 & 2.658 & 17.7461 & 0.0177 & 17.564 & 0.008 \\
333.8626 & 51.62510 & 324.357 & 5.312 & 424.997 & 9.040 & 17.6222 & 0.0178 & 17.329 & 0.023 \\
333.8692 & 51.62597 & 73.758 & 1.207 & 98.149 & 1.169 & 19.2302 & 0.0178 & 18.920 & 0.013 \\
333.8615 & 51.62311 & 372.171 & 6.085 & 475.846 & 5.671 & 17.4729 & 0.0178 & 17.206 & 0.013 \\
333.8502 & 51.62017 & 431.637 & 7.053 & 531.310 & 5.928 & 17.3120 & 0.0177 & 17.086 & 0.012 \\
333.8411 & 51.61808 & 203.417 & 3.340 & 306.930 & 2.502 & 18.1288 & 0.0178 & 17.682 & 0.009 \\
333.8412 & 51.61707 & 41.511 & 0.697 & 86.111 & 1.236 & 19.8543 & 0.0182 & 19.062 & 0.016 \\
333.8695 & 51.62316 & 62.754 & 1.026 & 96.130 & 2.453 & 19.4056 & 0.0177 & 18.943 & 0.028 \\
333.8394 & 51.61635 & 118.069 & 1.930 & 170.122 & 1.872 & 18.7194 & 0.0177 & 18.323 & 0.012 \\
333.8909 & 51.62732 & 71.476 & 1.171 & 118.268 & 0.951 & 19.2643 & 0.0178 & 18.718 & 0.009 \\
333.8475 & 51.61723 & 126.734 & 2.075 & 259.421 & 2.539 & 18.6425 & 0.0178 & 17.865 & 0.011 \\
333.8477 & 51.61646 & 62.639 & 1.438 & 129.725 & 1.576 & 19.4076 & 0.0249 & 18.617 & 0.013 \\
333.8564 & 51.61507 & 302.837 & 4.953 & 372.436 & 15.185 & 17.6967 & 0.0178 & 17.472 & 0.044 \\
333.8817 & 51.62058 & 19.869 & 0.641 & 126.375 & 1.695 & 20.6542 & 0.0350 & 18.646 & 0.015 \\
333.8834 & 51.61989 & 73.865 & 1.206 & 90.095 & 0.282 & 19.2287 & 0.0177 & 19.013 & 0.003 \\
333.8687 & 51.61631 & 67.061 & 1.098 & 125.294 & 2.347 & 19.3336 & 0.0178 & 18.655 & 0.020 \\
333.8793 & 51.61711 & 188.003 & 3.069 & 254.435 & 1.727 & 18.2144 & 0.0177 & 17.886 & 0.007 \\
333.8948 & 51.62009 & 105.422 & 1.721 & 209.766 & 5.197 & 18.8424 & 0.0177 & 18.095 & 0.027 \\
333.8571 & 51.61104 & 238.502 & 3.905 & 335.514 & 8.468 & 17.9560 & 0.0178 & 17.585 & 0.027 \\
333.8627 & 51.61000 & 143.542 & 2.344 & 186.070 & 1.843 & 18.5073 & 0.0177 & 18.226 & 0.011 \\
333.8721 & 51.61196 & 34.293 & 0.562 & 325.015 & 7.729 & 20.0617 & 0.0178 & 17.620 & 0.026 \\
333.8542 & 51.60796 & 116.508 & 1.907 & 164.458 & 3.252 & 18.7339 & 0.0178 & 18.360 & 0.021 \\
333.8882 & 51.61441 & 82.132 & 1.348 & 99.346 & 1.546 & 19.1135 & 0.0178 & 18.907 & 0.017 \\
333.8864 & 51.61390 & 315.944 & 5.154 & 443.606 & 12.715 & 17.6507 & 0.0177 & 17.282 & 0.031 \\
333.8739 & 51.61106 & 66.209 & 1.084 & 101.077 & 0.389 & 19.3475 & 0.0178 & 18.888 & 0.004 \\
333.9033 & 51.61763 & 46.447 & 0.761 & 87.190 & 0.681 & 19.7324 & 0.0178 & 19.049 & 0.008 \\
333.8468 & 51.60476 & 458.684 & 7.502 & 563.432 & 35.452 & 17.2460 & 0.0178 & 17.023 & 0.068 \\
333.8915 & 51.61423 & 400.284 & 6.528 & 585.933 & 8.291 & 17.3938 & 0.0177 & 16.980 & 0.015 \\
333.8728 & 51.60970 & 57.868 & 0.948 & 132.099 & 2.743 & 19.4937 & 0.0178 & 18.598 & 0.023 \\
333.8586 & 51.60625 & 115.194 & 2.162 & 149.760 & 1.943 & 18.7462 & 0.0204 & 18.461 & 0.014 \\
333.8466 & 51.60332 & 115.606 & 1.888 & 208.781 & 6.139 & 18.7423 & 0.0177 & 18.101 & 0.032 \\
333.8591 & 51.60568 & 102.400 & 2.639 & 127.805 & 1.732 & 18.8740 & 0.0280 & 18.633 & 0.015 \\
333.8528 & 51.60239 & 188.452 & 3.451 & 250.360 & 5.193 & 18.2118 & 0.0199 & 17.903 & 0.023 \\
333.8980 & 51.61246 & 48.621 & 0.800 & 375.469 & 3.497 & 19.6827 & 0.0179 & 17.463 & 0.010 \\
333.8502 & 51.60069 & 110.007 & 1.796 & 145.459 & 2.029 & 18.7962 & 0.0177 & 18.493 & 0.015 \\
333.8780 & 51.60693 & 21.690 & 0.359 & 101.762 & 1.130 & 20.5590 & 0.0179 & 18.881 & 0.012 \\
333.8698 & 51.60446 & 115.834 & 1.896 & 151.749 & 2.214 & 18.7402 & 0.0178 & 18.447 & 0.016 \\
333.8720 & 51.60456 & 111.682 & 1.830 & 159.642 & 2.871 & 18.7798 & 0.0178 & 18.392 & 0.020 \\
333.8955 & 51.60962 & 51.827 & 2.306 & 182.339 & 7.186 & 19.6133 & 0.0483 & 18.248 & 0.043 \\
333.8866 & 51.60743 & 56.752 & 0.936 & 93.150 & 2.122 & 19.5148 & 0.0179 & 18.977 & 0.025 \\
333.8966 & 51.60810 & 108.663 & 1.792 & 163.406 & 4.566 & 18.8096 & 0.0179 & 18.367 & 0.030 \\
333.8915 & 51.60527 & 119.178 & 1.968 & 203.693 & 1.820 & 18.7093 & 0.0179 & 18.127 & 0.010 \\
333.8876 & 51.60301 & 90.225 & 1.516 & 126.392 & 1.263 & 19.0114 & 0.0182 & 18.645 & 0.011 \\
333.9039 & 51.60638 & 93.369 & 1.524 & 155.881 & 1.180 & 18.9743 & 0.0177 & 18.418 & 0.008 \\
333.8525 & 51.59439 & 82.584 & 1.351 & 233.769 & 5.051 & 19.1075 & 0.0178 & 17.978 & 0.023 \\
333.8914 & 51.60243 & 222.542 & 3.716 & 306.799 & 2.898 & 18.0312 & 0.0181 & 17.683 & 0.010 \\
333.8985 & 51.60366 & 38.707 & 0.637 & 180.715 & 0.816 & 19.9302 & 0.0179 & 18.257 & 0.005 \\
333.8925 & 51.60199 & 189.532 & 3.188 & 294.720 & 1.533 & 18.2056 & 0.0183 & 17.726 & 0.006 \\
333.8758 & 51.59585 & 85.208 & 2.639 & 124.151 & 2.157 & 19.0736 & 0.0336 & 18.665 & 0.019 \\
333.8834 & 51.59720 & 152.412 & 2.489 & 237.063 & 1.259 & 18.4422 & 0.0177 & 17.963 & 0.006 \\
333.8761 & 51.59540 & 92.156 & 2.468 & 135.796 & 4.751 & 18.9885 & 0.0291 & 18.568 & 0.038 \\
333.8659 & 51.59150 & 118.065 & 1.927 & 136.789 & 4.042 & 18.7195 & 0.0177 & 18.560 & 0.032 \\
333.9069 & 51.60031 & 246.681 & 4.025 & 318.707 & 12.968 & 17.9194 & 0.0177 & 17.641 & 0.044 \\
333.8936 & 51.59652 & 203.626 & 3.323 & 292.643 & 2.288 & 18.1277 & 0.0177 & 17.734 & 0.008 \\
333.9099 & 51.59982 & 84.018 & 1.371 & 149.279 & 6.120 & 19.0888 & 0.0177 & 18.465 & 0.045 \\
333.8834 & 51.59317 & 136.061 & 2.220 & 422.654 & 3.137 & 18.5654 & 0.0177 & 17.335 & 0.008 \\
333.8653 & 51.58889 & 126.166 & 2.059 & 145.818 & 4.003 & 18.6474 & 0.0177 & 18.490 & 0.030 \\
333.8766 & 51.59134 & 99.135 & 1.619 & 160.447 & 1.229 & 18.9092 & 0.0177 & 18.386 & 0.008 \\
333.8895 & 51.59400 & 111.093 & 1.882 & 183.776 & 3.437 & 18.7855 & 0.0184 & 18.239 & 0.020 \\
333.8599 & 51.58722 & 93.070 & 1.670 & 309.019 & 3.852 & 18.9777 & 0.0195 & 17.675 & 0.014 \\
333.9082 & 51.59578 & 129.864 & 2.119 & 171.218 & 4.428 & 18.6160 & 0.0177 & 18.316 & 0.028 \\
333.8612 & 51.58502 & 29.541 & 0.486 & 95.211 & 0.682 & 20.2236 & 0.0179 & 18.953 & 0.008 \\
333.8753 & 51.58795 & 59.050 & 0.966 & 88.022 & 1.899 & 19.4717 & 0.0178 & 19.038 & 0.023 \\
333.8650 & 51.58549 & 170.538 & 2.787 & 299.823 & 2.691 & 18.3202 & 0.0177 & 17.708 & 0.010 \\
333.8899 & 51.59104 & 109.053 & 1.781 & 143.687 & 1.661 & 18.8057 & 0.0177 & 18.506 & 0.013 \\
333.9135 & 51.59565 & 237.387 & 4.118 & 312.985 & 9.229 & 17.9611 & 0.0188 & 17.661 & 0.032 \\
333.9034 & 51.59271 & 51.486 & 0.843 & 149.513 & 1.538 & 19.6205 & 0.0178 & 18.463 & 0.011 \\
333.9143 & 51.59436 & 167.645 & 2.739 & 270.198 & 7.402 & 18.3388 & 0.0177 & 17.821 & 0.030 \\
333.8803 & 51.58554 & 54.444 & 0.893 & 104.900 & 1.163 & 19.5599 & 0.0178 & 18.848 & 0.012 \\
333.8858 & 51.58586 & 107.347 & 1.751 & 167.434 & 4.305 & 18.8228 & 0.0177 & 18.340 & 0.028 \\
333.9063 & 51.59023 & 99.396 & 1.732 & 158.038 & 0.356 & 18.9063 & 0.0189 & 18.403 & 0.002 \\
333.8800 & 51.58320 & 235.592 & 3.843 & 298.899 & 4.676 & 17.9694 & 0.0177 & 17.711 & 0.017 \\
333.9119 & 51.58968 & 63.653 & 1.093 & 255.692 & 6.503 & 19.3902 & 0.0186 & 17.880 & 0.028 \\
333.8861 & 51.58383 & 210.915 & 3.448 & 281.916 & 2.729 & 18.0895 & 0.0177 & 17.774 & 0.011 \\
333.9030 & 51.58762 & 93.008 & 1.663 & 142.272 & 4.655 & 18.9785 & 0.0194 & 18.517 & 0.036 \\
333.9166 & 51.59061 & 570.913 & 9.314 & 583.215 & 6.627 & 17.0083 & 0.0177 & 16.985 & 0.012 \\
333.8882 & 51.58351 & 108.162 & 1.766 & 143.036 & 0.788 & 18.8146 & 0.0177 & 18.511 & 0.006 \\
333.8976 & 51.58560 & 60.762 & 1.003 & 235.798 & 6.200 & 19.4407 & 0.0179 & 17.968 & 0.029 \\
333.8842 & 51.58225 & 86.275 & 1.411 & 139.991 & 1.769 & 19.0601 & 0.0178 & 18.535 & 0.014 \\
333.8991 & 51.58522 & 115.919 & 1.900 & 161.240 & 4.510 & 18.7394 & 0.0178 & 18.381 & 0.030 \\
333.9175 & 51.58912 & 333.406 & 5.546 & 325.006 & 4.276 & 17.5923 & 0.0181 & 17.620 & 0.014 \\
333.9165 & 51.58857 & 473.393 & 7.914 & 504.742 & 3.432 & 17.2117 & 0.0181 & 17.142 & 0.007 \\
333.9161 & 51.58760 & 61.348 & 1.085 & 97.537 & 0.822 & 19.4303 & 0.0192 & 18.927 & 0.009 \\
333.8951 & 51.58256 & 97.594 & 1.595 & 126.811 & 4.253 & 18.9262 & 0.0177 & 18.642 & 0.036 \\
333.8635 & 51.57536 & 206.954 & 3.393 & 273.342 & 2.221 & 18.1101 & 0.0178 & 17.808 & 0.009 \\
333.9183 & 51.58750 & 186.917 & 3.054 & 272.895 & 8.753 & 18.2206 & 0.0177 & 17.810 & 0.035 \\
333.8975 & 51.58135 & 72.975 & 1.195 & 130.291 & 2.872 & 19.2418 & 0.0178 & 18.612 & 0.024 \\
333.9056 & 51.58206 & 174.399 & 2.844 & 221.167 & 0.559 & 18.2959 & 0.0177 & 18.038 & 0.003 \\
333.8714 & 51.57304 & 32.227 & 0.528 & 95.961 & 2.676 & 20.1292 & 0.0178 & 18.944 & 0.030 \\
333.8992 & 51.57794 & 76.711 & 1.252 & 101.699 & 2.943 & 19.1876 & 0.0177 & 18.881 & 0.031 \\
333.9250 & 51.58293 & 47.457 & 0.776 & 256.308 & 1.179 & 19.7090 & 0.0177 & 17.878 & 0.005 \\
333.8775 & 51.57212 & 480.377 & 7.847 & 523.658 & 12.017 & 17.1958 & 0.0177 & 17.102 & 0.025 \\
333.8968 & 51.57601 & 195.699 & 3.190 & 281.986 & 7.502 & 18.1708 & 0.0177 & 17.774 & 0.029 \\
333.8705 & 51.56987 & 83.183 & 1.361 & 95.526 & 1.804 & 19.0997 & 0.0178 & 18.949 & 0.020 \\
333.8895 & 51.57365 & 346.218 & 5.647 & 407.933 & 9.978 & 17.5514 & 0.0177 & 17.373 & 0.027 \\
333.8704 & 51.56821 & 90.433 & 1.478 & 132.973 & 2.548 & 19.0089 & 0.0178 & 18.590 & 0.021 \\
333.8920 & 51.57248 & 349.894 & 5.731 & 384.894 & 2.495 & 17.5399 & 0.0178 & 17.436 & 0.007 \\
333.8722 & 51.56730 & 237.881 & 3.883 & 263.802 & 3.926 & 17.9589 & 0.0177 & 17.847 & 0.016 \\
333.9114 & 51.57358 & 186.169 & 3.036 & 218.415 & 0.573 & 18.2250 & 0.0177 & 18.052 & 0.003 \\
333.9000 & 51.56972 & 59.823 & 0.979 & 106.811 & 2.047 & 19.4576 & 0.0178 & 18.828 & 0.021 \\
333.9111 & 51.57146 & 121.329 & 1.984 & 156.321 & 4.072 & 18.6899 & 0.0178 & 18.415 & 0.028 \\
333.9177 & 51.57290 & 140.309 & 2.297 & 221.847 & 4.905 & 18.5320 & 0.0178 & 18.035 & 0.024 \\
333.8949 & 51.56524 & 363.392 & 5.931 & 427.323 & 17.084 & 17.4988 & 0.0177 & 17.323 & 0.043 \\
333.9039 & 51.56664 & 171.609 & 2.801 & 225.722 & 2.814 & 18.3134 & 0.0177 & 18.016 & 0.014 \\
333.8972 & 51.56509 & 81.246 & 1.401 & 110.358 & 2.496 & 19.1253 & 0.0187 & 18.793 & 0.025 \\
333.8925 & 51.56384 & 159.179 & 2.983 & 200.471 & 5.194 & 18.3950 & 0.0203 & 18.145 & 0.028 \\
333.9004 & 51.56545 & 93.031 & 1.523 & 121.869 & 3.278 & 18.9782 & 0.0178 & 18.685 & 0.029 \\
333.8959 & 51.56398 & 45.051 & 0.737 & 136.750 & 3.529 & 19.7655 & 0.0178 & 18.560 & 0.028 \\
333.8844 & 51.56068 & 47.845 & 0.788 & 120.302 & 2.497 & 19.7001 & 0.0179 & 18.699 & 0.023 \\
333.8914 & 51.56222 & 60.500 & 0.988 & 90.122 & 0.900 & 19.4454 & 0.0177 & 19.013 & 0.011 \\
333.8962 & 51.56266 & 224.526 & 3.663 & 288.491 & 3.893 & 18.0216 & 0.0177 & 17.749 & 0.015 \\
333.8839 & 51.55960 & 418.313 & 6.828 & 465.160 & 9.220 & 17.3460 & 0.0177 & 17.231 & 0.022 \\
333.8914 & 51.56049 & 199.408 & 3.254 & 231.199 & 1.490 & 18.1504 & 0.0177 & 17.990 & 0.007 \\
333.9163 & 51.56306 & 83.792 & 1.367 & 89.935 & 2.534 & 19.0917 & 0.0177 & 19.015 & 0.031 \\
333.9293 & 51.56596 & 403.254 & 6.602 & 346.668 & 8.312 & 17.3858 & 0.0178 & 17.550 & 0.026 \\
333.9302 & 51.56561 & 45.043 & 4.193 & 95.185 & 0.583 & 19.7657 & 0.1011 & 18.953 & 0.007 \\
333.8810 & 51.55441 & 68.046 & 1.113 & 98.359 & 2.766 & 19.3178 & 0.0178 & 18.918 & 0.031 \\
333.9330 & 51.56611 & 394.489 & 6.456 & 524.258 & 16.239 & 17.4097 & 0.0178 & 17.101 & 0.034 \\
333.8891 & 51.55596 & 71.568 & 1.168 & 120.460 & 2.675 & 19.2630 & 0.0177 & 18.698 & 0.024 \\
333.9310 & 51.56474 & 65.054 & 1.065 & 114.586 & 0.204 & 19.3666 & 0.0178 & 18.752 & 0.002 \\
333.9170 & 51.56094 & 97.767 & 1.596 & 119.385 & 3.430 & 18.9243 & 0.0177 & 18.707 & 0.031 \\
333.8816 & 51.55207 & 95.004 & 1.816 & 220.151 & 5.556 & 18.9554 & 0.0208 & 18.043 & 0.027 \\
333.9265 & 51.56213 & 143.350 & 2.347 & 216.849 & 6.658 & 18.5088 & 0.0178 & 18.059 & 0.033 \\
333.8858 & 51.55282 & 162.631 & 2.660 & 155.350 & 2.499 & 18.3718 & 0.0178 & 18.421 & 0.017 \\
333.9243 & 51.56104 & 52.227 & 0.854 & 97.494 & 0.171 & 19.6050 & 0.0177 & 18.927 & 0.002 \\
333.9344 & 51.56015 & 269.061 & 4.403 & 407.470 & 9.789 & 17.8251 & 0.0178 & 17.375 & 0.026 \\
333.8855 & 51.54907 & 91.390 & 1.500 & 95.885 & 0.689 & 18.9975 & 0.0178 & 18.945 & 0.008 \\
333.8930 & 51.54973 & 393.105 & 6.416 & 368.053 & 6.279 & 17.4135 & 0.0177 & 17.485 & 0.019 \\
333.9261 & 51.55697 & 148.080 & 2.421 & 434.565 & 12.732 & 18.4735 & 0.0177 & 17.305 & 0.032 \\
333.9156 & 51.55301 & 44.868 & 0.734 & 94.480 & 2.966 & 19.7699 & 0.0178 & 18.961 & 0.034 \\
333.8997 & 51.54869 & 154.285 & 2.525 & 190.710 & 2.384 & 18.4290 & 0.0178 & 18.199 & 0.014 \\
333.8960 & 51.54787 & 174.181 & 2.844 & 444.452 & 6.984 & 18.2973 & 0.0177 & 17.280 & 0.017 \\
\end{tabular}\label{t:cat_j2215}
\tablenotetext{1}{AB magnitudes in the Lupton system, $m = m_{_0} - 2.5 \log b^\prime - (2.5 \log e) \sinh^{-1} (f/2b^\prime)$, using softening parameters $b^\prime = 0.242$ and 0.462 $\mu Jy$ for the $g$ and $i$ band, respectively, and zeropoint $m_{_0} = -48.6$.}
\tablenotetext{2}{The flux and magnitude errors represent the formal uncertainties. One should also add in quadrature the zeropoint calibration errors, which are 0.302 and 0.302 mag in $g$ and $i$ band, respectively.}
\end{center}
\end{table}

